X-Instruction: Aligning Language Model in Low-resource Languages with Self-curated Cross-lingual Instructions

Large language models respond well in high-resource languages like English but struggle in low-resource languages. It may arise from the lack of high-quality instruction following data in these languages. Directly translating English samples into these languages can be a solution but unreliable, leading to responses with translation errors and lacking language-specific or cultural knowledge. To address this issue, we propose a novel method to construct cross-lingual instruction following samples with instruction in English and response in low-resource languages. Specifically, the language model first learns to generate appropriate English instructions according to the natural web texts in other languages as responses. The candidate cross-lingual instruction tuning samples are further refined and diversified. We have employed this method to build a large-scale cross-lingual instruction tuning dataset on 10 languages, namely X-Instruction. The instruction data built using our method incorporate more language-specific knowledge compared with the naive translation method. Experimental results have shown that the response quality of the model tuned on X-Instruction greatly exceeds the model distilled from a powerful teacher model, reaching or even surpassing the ones of ChatGPT. In addition, we find that models tuned on cross-lingual instruction following samples can follow the instruction in the output language without further tuning.

==> tabs/four_benchmark_win_rate_on_three_languages.tex <==
\begin{table*}[thp]

\renewcommand\arraystretch{1.3}

\centering
\scriptsize

\setlength{\tabcolsep}{0.6mm}

 \begin{tabu}{l|cccc|cccc|cccc|cccc}
 
 \toprule[1.2pt]
  \multicolumn{1}{c}{ } & \multicolumn{4}{c}{\textbf{Vicuna}} & \multicolumn{4}{c}{\textbf{LIMA}} & \multicolumn{4}{c}{\textbf{WizardLM}} & \multicolumn{4}{c}{\textbf{Koala}} \\

  \cmidrule(r){2-5} \cmidrule(r){6-9} \cmidrule(r){10-13} \cmidrule(r){14-17} \noalign{\smallskip}

 \multicolumn{1}{c}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{bn}} & \multicolumn{1}{c}{\textbf{sw}} & \multicolumn{1}{c}{\textbf{ur}} & \multicolumn{1}{c}{ } & \multicolumn{1}{c}{\textbf{bn}} & \multicolumn{1}{c}{\textbf{sw}} & \multicolumn{1}{c}{\textbf{ur}} & \multicolumn{1}{c}{ } & \multicolumn{1}{c}{\textbf{bn}} & \multicolumn{1}{c}{\textbf{sw}} & \multicolumn{1}{c}{\textbf{ur}} & \multicolumn{1}{c}{ } & \multicolumn{1}{c}{\textbf{bn}} & \multicolumn{1}{c}{\textbf{sw}} & \multicolumn{1}{c}{\textbf{ur}} & \multicolumn{1}{c}{ } \\

  \cmidrule(r){2-4} \cmidrule(r){6-8} \cmidrule(r){10-12} \cmidrule(r){14-16} \noalign{\smallskip}
  
  \multicolumn{1}{c}{$\sim$\textsc{7b models}}& \multicolumn{3}{c}{\textbf{Win Rate $\%$}} & \multicolumn{1}{c}{\textbf{Avg}} & \multicolumn{3}{c}{\textbf{Win Rate $\%$}} & \multicolumn{1}{c}{\textbf{Avg}} & \multicolumn{3}{c}{\textbf{Win Rate $\%$}} & \multicolumn{1}{c}{\textbf{Avg}} & \multicolumn{3}{c}{\textbf{Win Rate $\%$}} & \multicolumn{1}{c}{\textbf{Avg}} \\

  
  

\midrule[0.8pt]
 $\text{Bactrian-X}_{\text{7B}+\text{Multilingual}}$

&$1.25$&$x$&$6.25$&$x$
&$0.33$&$32.67$&$3.42$&$12.14$
&$1.83$&$21.56$&$2.23$&$8.54$
&$1.72$&$24.14$&$3.03$&$9.63$ \\

 $\text{Bactrian-X}_{\text{7B}+\text{Monolingual}}$

&$45.00$&$56.25$&$57.50$&$52.92$
&$44.67$&$59.00$&$60.00$&$54.56$
&$30.28$&$42.66$&$45.87$&$39.60$
&$24.44$&$33.33$&$31.67$&$29.81$ \\


 $\text{X-Instruct}_{\text{7B}}$                        

&$61.25$&$60.00$&$60.00$&$60.42$
&$61.67$&$67.33$&$77.00$&$68.67$
&$33.94$&$51.83$&$56.42$&$47.40$
&$37.22$&$37.22$&$56.67$&$43.70$ \\


$\text{X-Instruct}_{\text{7B}}(\text{zero-shot})$                        

&$42.50$&$42.50$&$58.75$&$47.92$
&$51.00$&$58.33$&$63.33$&$57.55$
&$32.57$&$41.74$&$48.17$&$40.83$
&$28.16$&$38.51$&$41.95$&$36.21$ \\

% GPT-4 Score
\midrule[0.8pt]
\multicolumn{1}{c}{ }& \multicolumn{3}{c}{\textbf{GPT-4 Score}} & \multicolumn{1}{c}{\textbf{Avg}} & \multicolumn{3}{c}{\textbf{GPT-4 Score}} & \multicolumn{1}{c}{\textbf{Avg}} & \multicolumn{3}{c}{\textbf{GPT-4 Score}} & \multicolumn{1}{c}{\textbf{Avg}} & \multicolumn{3}{c}{\textbf{GPT-4 Score}} & \multicolumn{1}{c}{\textbf{Avg}} \\
\midrule[0.8pt]
 $\text{Bactrian-X}_{\text{7B}+\text{Multilingual}}$
&$0.19$&$x$&$0.50$&$x$ 
&$0.04$&$3.42$&$0.51$&$1.32$
&$0.16$&$2.23$&$0.35$&$0.91$
&$0.19$&$3.03$&$0.33$&$1.18$ \\


 $\text{Bactrian-X}_{\text{7B}+\text{Monolingual}}$
&$4.81$&$8.05$&$6.89$&$6.53$ 
&$3.87$&$6.88$&$5.33$&$5.36$
&$3.23$&$5.37$&$4.63$&$4.41$ 
&$2.94$&$5.34$&$4.08$&$4.12$ \\


 $\text{X-Instruct}_{\text{7B}}$                        
&$7.34$&$8.04$&$6.99$&$7.70$
&$5.83$&$7.84$&$7.82$&$7.16$ 
&$4.02$&$6.61$&$6.18$&$5.60$
&$4.88$&$6.22$&$6.66$&$5.92$\\

$\text{X-Instruct}_{\text{7B}}(\text{zero-shot})$                        
&$5.22$&$6.36$&$6.61$&$6.06$
&$4.64$&$6.74$&$6.42$&$5.93$ 
&$3.81$&$5.85$&$5.27$&$4.98$
&$3.74$&$5.36$&$5.37$&$4.82$\\



\midrule[0.8pt]
\midrule[0.8pt]

\multicolumn{1}{c}{$\sim$\textsc{13b models}}& \multicolumn{3}{c}{\textbf{Win Rate $\%$}} & \multicolumn{1}{c}{\textbf{Avg}} & \multicolumn{3}{c}{\textbf{Win Rate $\%$}} & \multicolumn{1}{c}{\textbf{Avg}} & \multicolumn{3}{c}{\textbf{Win Rate $\%$}} & \multicolumn{1}{c}{\textbf{Avg}} & \multicolumn{3}{c}{\textbf{Win Rate $\%$}} & \multicolumn{1}{c}{\textbf{Avg}} \\

  
  

\midrule[0.8pt]
 $\text{Bactrian-X}_{\text{7B}+\text{Multilingual}}$

&$1.25$&$x$&$6.25$&$x$
&$0.33$&$32.67$&$3.42$&$12.14$
&$1.83$&$21.56$&$2.23$&$8.54$
&$1.72$&$24.14$&$3.03$&$9.63$ \\






 $\text{Bactrian-X}_{\text{7B}+\text{Monolingual}}$

&$45.00$&$56.25$&$57.50$&$52.92$
&$44.67$&$59.00$&$60.00$&$54.56$
&$30.28$&$42.66$&$45.87$&$39.60$
&$24.44$&$33.33$&$31.67$&$29.81$ \\




 $\text{X-Instruct}_{\text{7B}}$                        

&$61.25$&$60.00$&$60.00$&$60.42$
&$61.67$&$67.33$&$77.00$&$68.67$
&$33.94$&$51.83$&$56.42$&$47.40$
&$37.22$&$37.22$&$56.67$&$43.70$ \\


$\text{X-Instruct}_{\text{7B}}(\text{zero-shot})$                        

&$42.50$&$42.50$&$58.75$&$47.92$
&$51.00$&$58.33$&$63.33$&$57.55$
&$32.57$&$41.74$&$48.17$&$40.83$
&$28.16$&$38.51$&$41.95$&$36.21$ \\

% GPT-4 Score
\midrule[0.8pt]
\multicolumn{1}{c}{ }& \multicolumn{3}{c}{\textbf{GPT-4 Score}} & \multicolumn{1}{c}{\textbf{Avg}} & \multicolumn{3}{c}{\textbf{GPT-4 Score}} & \multicolumn{1}{c}{\textbf{Avg}} & \multicolumn{3}{c}{\textbf{GPT-4 Score}} & \multicolumn{1}{c}{\textbf{Avg}} & \multicolumn{3}{c}{\textbf{GPT-4 Score}} & \multicolumn{1}{c}{\textbf{Avg}} \\
\midrule[0.8pt]
 $\text{Bactrian-X}_{\text{7B}+\text{Multilingual}}$
&$0.19$&$x$&$0.50$&$x$ 
&$0.04$&$3.42$&$0.51$&$1.32$
&$0.16$&$2.23$&$0.35$&$0.91$
&$0.19$&$3.03$&$0.33$&$1.18$ \\


 $\text{Bactrian-X}_{\text{7B}+\text{Monolingual}}$
&$4.81$&$8.05$&$6.89$&$6.53$ 
&$3.87$&$6.88$&$5.33$&$5.36$
&$3.23$&$5.37$&$4.63$&$4.41$ 
&$2.94$&$5.34$&$4.08$&$4.12$ \\


 $\text{X-Instruct}_{\text{7B}}$                        
&$7.34$&$8.04$&$6.99$&$7.70$
&$5.83$&$7.84$&$7.82$&$7.16$ 
&$4.02$&$6.61$&$6.18$&$5.60$
&$4.88$&$6.22$&$6.66$&$5.92$\\

$\text{X-Instruct}_{\text{7B}}(\text{zero-shot})$                        
&$5.22$&$6.36$&$6.61$&$6.06$
&$4.64$&$6.74$&$6.42$&$5.93$ 
&$3.81$&$5.85$&$5.27$&$4.98$
&$3.74$&$5.36$&$5.37$&$4.82$\\
 

\bottomrule[1.2pt]
\end{tabu}
\vspace{-2mm}

\caption{\label{tab:win_rates_all} The win rates to ChatGPT and average scores of different multilingual models evaluated by GPT-4. 
}

\vspace{-2mm}

\end{table*}

==> tabs/win_rates_all.tex <==
\begin{table*}[thp]

\renewcommand\arraystretch{1.1}

\centering
\scriptsize

\setlength{\tabcolsep}{0.6mm}

 \begin{tabu}{l|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|c}
 
 \toprule[1.2pt]
  % \multicolumn{1}{c}{ } & \multicolumn{6}{c}{\textbf{Medium}} & \multicolumn{6}{c}{\textbf{Low}} &\\
  % \cmidrule(r){2-7}  \cmidrule(r){8-13} \noalign{\smallskip}
  
  \multicolumn{1}{c}{ } & \multicolumn{2}{c}{\textbf{fi}} & \multicolumn{2}{c}{\textbf{id}} & \multicolumn{2}{c}{\textbf{th}} & \multicolumn{2}{c}{\textbf{tr}} & \multicolumn{2}{c}{\textbf{vi}} & \multicolumn{2}{c}{\textbf{bn}} & \multicolumn{2}{c}{\textbf{hi}} & \multicolumn{2}{c}{\textbf{sw}} & \multicolumn{2}{c}{\textbf{ta}} & \multicolumn{2}{c}{\textbf{ur}} \\
  \cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} \cmidrule(r){10-11} \cmidrule(r){12-13} \cmidrule(r){14-15} \cmidrule(r){16-17} \cmidrule(r){18-19} \cmidrule(r){20-21} \noalign{\smallskip}
  
\multicolumn{1}{c}{\textbf{Model}}& \textbf{W}&\textbf{S}& \textbf{W}&\textbf{S}& \textbf{W}&\textbf{S}& \textbf{W}&\textbf{S}& \textbf{W}&\textbf{S}& \textbf{W}&\textbf{S} & \textbf{W}&\textbf{S} & \textbf{W}&\textbf{S} & \textbf{W}&\textbf{S} & \textbf{W}&\textbf{S} &\multicolumn{1}{c}{\textbf{Avg}}\\


% Vicuna
\midrule[0.8pt]
\multicolumn{1}{c}{ } &\multicolumn{20}{c}{\textit{Vicuna}} & \multicolumn{1}{c}{ }\\
\midrule[0.8pt]
 $\text{Bactrian-X}_{\text{7B}+\text{Multilingual}}$
 &x&x&x&x&0.00&0.10&32.50&1.76&x&x&1.25&0.19&x&x&x&x&x&x&6.25&0.50&0.64\\


 $\text{Bactrian-X}_{\text{7B}+\text{Monolingual}}$
&41.25&7.38&46.25&7.70&45.00&6.92&58.75&6.51&55.00&7.67&45.00&4.81&72.50&6.61&56.25&8.05&42.50&2.74&57.50&6.89&6.53 \\


 $\text{X-Instruct}_{\text{7B}}$                        
&42.50&7.87&50.00&8.25&51.25&7.47&67.50&7.41&65.00&8.51&61.25&7.34&77.50&8.04&60.00&8.04&80.00&7.08&60.00&6.99&7.70\\


 % \cdashline{1-14}
 $\text{X-Instruct}_{\text{7B}}(\text{zero-shot})$                        
&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&42.50&5.22&\text{-}&\text{-}&42.50&6.36&\text{-}&\text{-}&58.75&6.61&6.06\\



% LIMA
 \midrule[0.8pt]
\multicolumn{1}{c}{ } &\multicolumn{20}{c}{\textit{LIMA}} & \multicolumn{1}{c}{ }\\
\midrule[0.8pt]
 $\text{Bactrian-X}_{\text{7B}+\text{Multilingual}}$        
&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&0.33&0.04&\text{-}&\text{-}&32.67&3.42&\text{-}&\text{-}&5.67&0.51&1.32\\
 $\text{Bactrian-X}_{\text{7B}+\text{Monolingual}}$        &\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&44.67&3.87&\text{-}&\text{-}&59.00&6.88&\text{-}&\text{-}&60.00&5.33&5.36\\
 $\text{X-Instruct}_{\text{7B}}$                        &\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&61.67&5.83&\text{-}&\text{-}&67.33&7.84&\text{-}&\text{-}&77.00&7.82&7.16\\
 % \cdashline{1-14}
 $\text{X-Instruct}_{\text{7B}}(\text{zero-shot})$                       &\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&51.00&4.64&\text{-}&\text{-}&58.33&6.74&\text{-}&\text{-}&63.33&6.42&5.93\\


% WizardLM
 \midrule[0.8pt]
\multicolumn{1}{c}{ } &\multicolumn{20}{c}{\textit{WizardLM}} & \multicolumn{1}{c}{ }\\
\midrule[0.8pt]
 $\text{Bactrian-X}_{\text{7B}+\text{Multilingual}}$
&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&1.83&0.16&\text{-}&\text{-}&21.56&2.23&\text{-}&\text{-}&4.13&0.35&0.91\\
 $\text{Bactrian-X}_{\text{7B}+\text{Monolingual}}$        &\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&30.28&3.23&\text{-}&\text{-}&42.66&5.37&\text{-}&\text{-}&45.87&4.63&4.41\\
 $\text{X-Instruct}_{\text{7B}}$                        &\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&33.94&4.02&\text{-}&\text{-}&51.83&6.61&\text{-}&\text{-}&56.42&6.18&5.60\\
 % \cdashline{1-14}
 $\text{X-Instruct}_{\text{7B}}(\text{zero-shot})$                       &\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&32.57&3.81&\text{-}&\text{-}&41.74&5.85&\text{-}&\text{-}&48.17&5.27&4.98\\



% Koala
\midrule[0.8pt]
\multicolumn{1}{c}{ } &\multicolumn{20}{c}{\textit{Koala}} & \multicolumn{1}{c}{ }\\
\midrule[0.8pt]
 $\text{Bactrian-X}_{\text{7B}+\text{Multilingual}}$ &\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&1.72&0.19&\text{-}&\text{-}&24.14&3.03&\text{-}&\text{-}&2.87&0.33&1.18\\
 $\text{Bactrian-X}_{\text{7B}+\text{Monolingual}}$        &\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&24.44&2.94&\text{-}&\text{-}&33.33&5.34&\text{-}&\text{-}&31.67&4.08&4.12\\
 $\text{X-Instruct}_{\text{7B}}$                        &\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&37.22&4.88&\text{-}&\text{-}&37.22&6.22&\text{-}&\text{-}&56.67&6.66&5.92\\
 % \cdashline{1-14}
 $\text{X-Instruct}_{\text{7B}}(\text{zero-shot})$                       &\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&\text{-}&28.16&3.74&\text{-}&\text{-}&38.51&5.36&\text{-}&\text{-}&41.95&5.37&4.82\\








 
% \midrule[0.8pt]
% \multicolumn{14}{c}{\textit{Cross-lingual Evaluation}} \\
% \midrule[0.8pt]
 % $\text{M}_{0}$                        & 50.5 & 189.6 & 50.5 & 189.6& 50.5 & 189.6& 50.5 & 189.6& 50.5 & 189.6& 50.5 & 189.6 & 189.6\\
% \midrule[0.8pt]
% \multicolumn{14}{c}{\textit{Zero-shot Multilingual Evaluation}} \\
% \midrule[0.8pt]
 
 

\bottomrule[1.2pt]
\end{tabu}
\vspace{-2mm}

\caption{\label{tab:win_rates_all} The win rates to ChatGPT and average scores of different multilingual models evaluated by GPT-4. 
}

\vspace{-2mm}

\end{table*}
